Truth in Web Mining: Measuring the Profitability and Cost of Cryptominers as a Web Monetization Model

The recent advances of web-based cryptomining libraries along with the whopping market value of cryptocoins have convinced an increasing number of publishers to switch to web mining as a source of monetization for their websites. The conditions could not be better nowadays: the inevitable arms race between adblockers and advertisers is at its peak with publishers caught in the crossfire. But, can cryptomining be the next primary monetization model in the post advertising era of free Internet? In this paper, we respond to this exact question. In particular, we compare the profitability of cryptomining and advertising to assess the most advantageous option for a content provider. In addition, we measure the costs imposed to the user in each case with regards to power consumption, resources utilization, network traffic, device temperature and user experience. Our results show that cryptomining can surpass the profitability of advertising under specific circumstances, however users need to sustain a significant cost on their devices.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Binded with the whopping values of cryptocoins, cryptomining enjoys nowadays a steadily increasing adoption 
by service providers. More and more publishers choose web mining for monetizing their websites in an attempt 
to abandon the sinking boat of digital advertising. But can cryptomining become a reliable alternative for the 
next day of free Internet?

To respond to this exact question, in this paper we compare the profitability of ads and cryptomining. In addition,
by collecting a large dataset of miner-supported websites we compare the costs of these two monetization 
models on the user side. Results of our study show that for the average duration of a website visit, ads 
are $5.5\times$ more profitable than cryptomining for a publisher. However, they can gain higher revenues with 
cryptomining if the visitor remains in the website for long ($>5.3$ minutes depending on the user's device). 
Furthermore, the increased resource utilization (59x more CPU utilization, additional 
network activity of 1 Kbit per second) force the visitor's system to sustain a heavy load that
has a significant impact on the overall system's condition (it operates in 52.8\% higher temperature and 
consumes 2.08x more energy). In summary, we see that cryptomining can indeed be considered as 
an alternative monetization method for publishers but it is unable to replace the current advertising model. 
